Three Quantization Regimes for ReLU Networks

We establish the fundamental limits in the approximation of Lipschitz functions by deep ReLU neural networks with finite-precision weights. Specifically, three regimes, namely under-, over-, and proper quantization, in terms of minimax approximation error behavior as a function of network weight precision, are identified. This is accomplished by deriving nonasymptotic tight lower and upper bounds on the minimax approximation error. Notably, in the proper-quantization regime, neural networks exhibit memory-optimality in the approximation of Lipschitz functions. Deep networks have an inherent advantage over shallow networks in achieving memory-optimality. We also develop the notion of depth-precision tradeoff, showing that networks with high-precision weights can be converted into functionally equivalent deeper networks with low-precision weights, while preserving memory-optimality. This idea is reminiscent of sigma-delta analog-to-digital conversion, where oversampling rate is traded for resolution in the quantization of signal samples. We improve upon the best-known ReLU network approximation results for Lipschitz functions and describe a refinement of the bit extraction technique which could be of independent general interest.

==> chapter/bounded_weight.tex <==
%!TEX root = ../draft_quantized_weight_networks.tex

\section{Bounded weight} % (fold)
\label{sec:bounded_weight}
	We can realize a network with certain weight, by a deeper network with a smaller weight with the following proposition.

	\begin{lemma}
		Suppose Let $d,W, L \in \mathbb{N}$, $B \in \mathbb{R}$, then for any positive number $\hat{B} \leq B $ and integer $\hat{L} \geq L$ such that $( B W )^{\hat{L} - L} ( \frac{\hat{B}}{B} )^{\hat{L}} \geq 1$, we have 
		\begin{equation*}
			\mathcal{R} ( d,W,L, B ) \subseteq \mathcal{R} ( d, 2W, \hat{L}, \hat{B} ).
		\end{equation*}

		\begin{proof}
			\todo{proof calculate the covering number required for this realization, still doable I suppose... }
		\end{proof}
	\end{lemma}
% section bounded_weight (end)
